Random Feature Expansions for Deep Gaussian Processes

The composition of multiple Gaussian Processes as a Deep Gaussian Process (DGP) enables a deep probabilistic nonparametric approach to flexibly tackle complex machine learning problems with sound quantification of uncertainty. Existing inference approaches for DGP models have limited scalability and are notoriously cumbersome to construct. In this work, we introduce a novel formulation of DGPs based on random feature expansions that we train using stochastic variational inference. This yields a practical learning framework which significantly advances the state-of-the-art in inference for DGPs, and enables accurate quantification of uncertainty. We extensively showcase the scalability and performance of our proposal on several datasets with up to 8 million observations, and various DGP architectures with up to 30 hidden layers.

==> gps.tex <==
\subsection{Gaussian Processes}

%% \input{figures/diagram.tex}


%% \noteEB{Equations are part of the text so should be followed by punctuation when necessary.}
Consider a supervised learning scenario where a set of input vectors $X = [\xvect_1, \ldots, \xvect_\nobs]^{\top}$ is associated with a set of (possibly multivariate) labels $Y = [\yvect_1, \ldots, \yvect_\nobs]^{\top}$, where $\xvect_i \in R^{D_{\mathrm{in}}}$ and $\yvect_i \in R^{D_{\mathrm{out}}}$.
We assume that there is an underlying function $f_o(\xvect_i)$ characterizing a mapping from the inputs to a latent (unobserved) representation, and that the labels are a realization of some probabilistic process $p(y_{io} | f_o(\xvect_i))$ which is based on this latent representation.

GP models assume a nonparametric form for the latent functions.
%% Unlike parametric approaches, where $f_o(\xvect_i)$ is assumed to belong to a class of functions with a specific parametric form (e.g., linear combination of basis functions), in nonparametric approaches $f_o(\xvect_i)$ is assumed to belong to a much richer class of functions.
%% GPs \citep{Rasmussen06} do so by defining a prior distribution over functions $f_o(\xvect_i)$, and through the application of Bayesian inference techniques the aim is to learn the posterior distribution over functions, along with any parameters specifying the class of modeled functions, after data are observed, with the ultimate goal of making predictions that take into account all the functions in the class that are compatible with the observed data.
%% The added flexibility in defining a nonparametric prior over functions is controlled by a form of regularization stemming from the use of probabilistic techniques to learn GPs.
Formally, GPs are a collection of random variables such that any subset of these are jointly Gaussian distributed \citep{Rasmussen06}.
In GPs, the covariance between variables at different locations, say $f_o(\xvect_i)$ and $f_o(\xvect_j)$, is modeled using a covariance function $k(\xvect_i, \xvect_j | \thetavect)$ parameterized via a set of parameters $\thetavect$.
%% For the sake of simplicity, we assume that the covariance parameters are the same across the different outputs of the model, but this assumption can be relaxed.
A typical example of a covariance function, which we  use throughout the paper, 
is the Radial Basis Function (RBF) covariance with Automatic Relevance Determination (ARD)~\citep{Mackay94}
\begin{equation} \label{eq:kernel:rbf:ard}
%% k(\xvect_i, \xvect_j | \thetavect) = 
%% \sigma^2 \exp\left[-\frac{1}{2} (\xvect_i - \xvect_j)^{\top} \Lambda^{-1} (\xvect_i - \xvect_j) \right] \text{.}
k(\xvect, \xvect^{\prime} | \thetavect) = 
\sigma^2 \exp\left[-\frac{1}{2} (\xvect - \xvect^{\prime})^{\top} \Lambda^{-1} (\xvect - \xvect^{\prime}) \right] \text{.}
\end{equation}
The parameter set $\thetavect$ comprises the marginal variance of the GP $\sigma^2$, and $\Lambda = \diag(l_1^2, \ldots, l_d^2)$, with the $l_i$'s interpreted as lengthscale parameters along each of the dimensions of the input domain.

Another kernel that we will employ throughout the paper is the arc-cosine kernel of order $p$, which is defined as:
\begin{equation} \label{eq:kernel:arccosine:ard}
k_{\text{arc}}^{(p)}(\xvect, \xvect^{\prime}) = 
\frac{1}{\pi} \left\| \xvect \right\|^p \left\|\xvect^{\prime}\right\|^p J_p\left( \cos^{-1}\left( \frac{\xvect^{\top} \xvect^{\prime}}{\| \xvect \| \| \xvect^{\prime}\|} \right) \right) 
\quad \text{with}
\end{equation}
%% \begin{equation} \label{eq:kernel:arccosine:ard}
%% k_{\text{arc}}^{(p)}(\xvect, \xvect^{\prime} | \thetavect) = 
%% \frac{\sigma^2}{\pi} \left\| \Lambda^{-\frac{1}{2}} \xvect \right\|^p \left\| \Lambda^{-\frac{1}{2}} \xvect^{\prime}\right\|^p J_p\left( \cos^{-1}\left( \frac{\xvect^{\top} \Lambda^{-1} \xvect^{\prime}}{\| \Lambda^{-\frac{1}{2}} \xvect \| \| \Lambda^{-\frac{1}{2}} \xvect^{\prime}\|} \right) \right)
%% \end{equation}
with
\begin{equation}
J_p(\alpha) = (-1)^p (\sin \alpha)^{2p + 1} \left(\frac{1}{\sin\alpha} \frac{\partial}{\partial \alpha}\right)^p \left( \frac{\pi - \alpha}{\sin \alpha} \right) \text{.}
\end{equation}


%% Given a dataset of $\nobs$ observations, learning and predicting require operations involving the $\nobs \times \nobs$ covariance matrix $K$ with entries $k_{ij} = k(\xvect_i, \xvect_j | \thetavect)$.
%% %% Optimizing or inferring $\thetavect$ and making predictions for new input vectors $\xvect_*$ 
%% %% only require operations involving the $N \times N$ covariance matrix $K$ with entries $k_{ij} = k(\xvect_i, \xvect_j | \thetavect)$.
%% Denote by $F$ the set of latent variables with entries $f_{io} = f_o(\xvect_i)$, and let $p(Y | F)$ be the conditional likelihood.
%% Optimization or inference of covariance parameters requires repeatedly calculating 
%% $$
%% p(Y | \thetavect, X) = \int p(Y | F) p(F | \thetavect, X) dF \text{,}
%% $$
%% whereas carrying out predictions for a new text point $\xvect_*$ requires solving
%% \begin{eqnarray}
%% p(\yvect_* | Y, \thetavect, X, \xvect_*) & = & \int p(\yvect_* | \fvect_*) p(\fvect_* | F, \thetavect, X, \xvect_*) \times \nonumber \\ 
%% & & \quad p(F | Y, \thetavect, X) d\fvect_* dF \nonumber \text{.}
%% \end{eqnarray}

Denote by $F$ the set of latent variables with entries $f_{io} = f_o(\xvect_i)$, and let $p(Y | F)$ be the conditional likelihood.
Given a dataset of $\nobs$ observations, we aim to optimize or infer covariance parameters that requires repeated evaluation of the marginal likelihood $p(Y | X, \thetavect)$.
After that, we wish to carry out predictions for a new test point $\xvect_*$ by evaluating $p(\yvect_* | Y, X, \xvect_*, \thetavect)$.
There are two main difficulties in dealing with these tasks.
First, in the case of a non-Gaussian likelihood $p(Y | F)$, the marginal likelihood and the predictive probability are analytically intractable.
Secondly, even in the case of a Gaussian likelihood where these are computable, the GP prior introduces the need to solve algebraic operations 
  with a computational cost of $O(\nobs^3)$. This poses a scalability issue for GPs that requires resorting to approximations. %problem is particularly acute in the case of large $\nobs$, and we are going to employ a spectral approximation to the covariance to reduce this complexity.
%% The matrix operations are $\log|K|$ and the solution of linear systems involving $K$.
%% Several techniques have been proposed to deal with these issues; reviewing them here is beyond the scope of this work, so we refer the reader to \citep{Opper00,Opper09,Murray10b} for works that deal with non-Gaussian likelihoods, and to 
%% \citep{Csato02,Candela05,Hensman13} for works dealing with problems having large $\nobs$.
%% We also note recent work that has addressed both problems simultaneously \citep{Hensman15,Dezfouli15}.
%



%% \subsection{GPs with random Fourier features}
%% In this work, we focus on the so-called spectral approximation of GPs.
%% Appealing to Bochner's theorem, any continuous shift-invariant normalized covariance function $k(\xvect_i, \xvect_j) = k(\xvect_i - \xvect_j)$ is positive definite if and only if it can be rewritten as the Fourier transform of a non-negative measure $p(\omegavect)$ \citep{Rahimi08}.
%% Denoting the angular frequencies by $\omegavect$, while assigning $\iota = \sqrt{-1}$ and $\deltavect = \xvect_i - \xvect_j$, in the case of the RBF covariance detailed in equation~\ref{eq:kernel:rbf:ard}, this yields:
%% $$
%% k(\deltavect | \thetavect) = \sigma^2 \int p(\omegavect) \exp\left(\iota \deltavect^{\top} \omegavect \right) d\omegavect \text{,}
%% $$
%% with a corresponding non-negative measure $p(\omegavect) = \norm\left(\zerovect, \Lambda^{-1} \right)$.
%% Because the covariance function and the non-negative measures are real, we can drop the unnecessary complex part of the argument of the expectation, keeping $\cos(\deltavect^{\top} \omegavect) = \cos((\xvect_i - \xvect_j)^{\top} \omegavect)$ that can be rewritten as
%% $\cos(\xvect_i^{\top} \omegavect) \cos(\xvect_j^{\top} \omegavect) + \sin(\xvect_i^{\top} \omegavect) \sin(\xvect_j^{\top} \omegavect)$.
%% % Note that an alternative representation using only cosines can be found by introducing a uniformly distributed phase term \citep{Rahimi08,Gal16}.

%% The importance of the expansion above is that it allows us to interpret the covariance function as an expectation that can be estimated using Monte Carlo.
%% Defining $\zvect(\xvect | \omegavect) = [\cos(\xvect^{\top} \omegavect), \sin(\xvect^{\top} \omegavect)]^{\top}$, 
%% the covariance function can be approximated by the following (unbiased) Monte Carlo estimate
%% $$
%% k(\xvect_i, \xvect_j | \thetavect) \approx \frac{\sigma^2}{N_{\mathrm{RFF}}} \sum_{r=1}^{N_{\mathrm{RFF}}} \zvect(\xvect_i | \tilde{\omegavect}_r)^{\top} \zvect(\xvect_j | \tilde{\omegavect}_r) \text{,}
%% $$
%% with $\tilde{\omegavect}_{r} \sim p(\omegavect)$.

%% %% In practice, this expansion leads to an explicit representation of the mapping induced by the choice of covariance function.
%% This has an important practical implication, as it provides the means to access an approximate explicit representation of the mapping induced by the covariance function that, in the RBF case, we know is infinite dimensional~\citep{Shawe-Taylor04}.
%% In consequence, instead of defining a learning problem in the space induced by the covariance function, it is possible to reformulate the problem in an explicit finite representation given by the expansion using random Fourier features.
%% Defining $\Omega$ to be $[\tilde{\omegavect}_1, \ldots, \tilde{\omegavect}_{N_{\mathrm{RFF}}}]$, this representation suggests transforming the inputs into a new design matrix as follows:
%% $$
%% \Phi = \sqrt{\frac{\sigma^2}{N_{\mathrm{RFF}}}} \left[ \cos\left(X \Omega\right), \sin\left(X \Omega\right) \right] \text{,}
%% $$
%% where sine and cosine are applied element-wise to their argument.
%% %% $$
%% %% \Phi = \left[\sqrt{\frac{\sigma^2}{N_{\mathrm{RFF}}}} \cos\left(X \Omega\right), \sqrt{\frac{\sigma^2}{N_{\mathrm{RFF}}}} \sin\left(X \Omega\right) \right] \text{.}
%% %% $$
%% The original GP model is now ``linearized'' and can be treated as a standard linear model with a design matrix $\Phi$.
%% Therefore, considering a set of weights in matrix form $W$, %$W = [\wvect_1, \ldots, \wvect_o]$, 
%% the latent functions can be expressed as $F = \Phi W$.
%% The columns of $W$ are the coefficients of linear combinations of the random Fourier features to obtain the latent functions modeling the output labels.
%% Analyzing the mean and the covariance of a given latent function, in the case where $w_{io} \sim \norm(w_{io} | 0, 1)$, we can easily verify that the mean and covariance of the latent functions are zero and $\Phi \Phi^{\top} \approx K$, respectively, as we sought.
%% %% we see that
%% %% $$
%% %% \E[F_{\cdot i}] = \E[\Phi W_{\cdot i}] = \Phi \E[W_{\cdot i}] = \zerovect \text{,}
%% %% $$
%% %% and 
%% %% \begin{align*}
%% %% \mathrm{cov}[F_{\cdot i}] &= \E[\Phi W_{\cdot i} W_{\cdot i}^{\top} \Phi^{\top}] = \Phi \E[W_{\cdot i} W_{\cdot i}^{\top}] \Phi^{\top} \\
%% %% &= \Phi \Phi^{\top} \approx K \text{,}
%% %% \end{align*}
%% %% as we sought.
%% %%
%% %% We make two important remarks here. 
%% %% First, the prior over $W_{\cdot i}$ has to be $\norm(W_{\cdot i} | \zerovect, I)$ if we want to obtain the desired GP approximation.
%% %% Second, we observe that the usual practice of stacking a vector of ones to the design matrix to account for a nonzero constant mean in the linear model has the undesired effect of changing the covariance.
%% %% To see this, define
%% %% $$
%% %% \tilde{\Phi} = \left[\onesvect, \sqrt{\frac{\sigma^2}{N_{\mathrm{RFF}}}} \cos\left(X \Omega\right), \sqrt{\frac{\sigma^2}{N_{\mathrm{RFF}}}} \sin\left(X \Omega\right) \right]
%% %% $$
%% %% Then 
%% %% \begin{eqnarray}
%% %% \mathrm{cov}[F_{\cdot i}] & = & \E[\tilde{\Phi} W_{\cdot i} W_{\cdot i}^{\top} \tilde{\Phi}^{\top}] = \tilde{\Phi} \E[W_{\cdot i} W_{\cdot i}^{\top}] \tilde{\Phi}^{\top} \nonumber \\
%% %% & = & \tilde{\Phi} \tilde{\Phi}^{\top} = \Phi \Phi^{\top} + \onesvect \onesvect^{\top} \approx K + \onesvect \onesvect^{\top} \text{.}
%% %% \end{eqnarray}
%% %% Given that we want to impose a specific covariance on our latent functions, we avoid introducing a nonzero mean by stacking a vector of ones to our design matrix.
%% %%
%% %% In the case of a regression model with a Gaussian likelihood, it is possible to obtain the posterior over $W$ analytically and integrate out $W$ to make predictions.
%% %% The mean of the posterior over $W$, for example, turns out to be the standard regularized least square estimator; the computational advantage is that this turns the original $O(N^3)$ problem into $O(N_{\mathrm{RFF}}^3)$.
%% The approximation turns the original $O(\nobs^3)$ learning and prediction problems into $O(N_{\mathrm{RFF}}^3)$, as $K$ is approximated by $\Phi \Phi^{\top}$ that has rank $2 N_{\mathrm{RFF}}$.
%% Various results have been established on the accuracy of the random Fourier feature approximation (see, e.g., \citet{Rahimi08}).


==> intro_old.tex <==
\section{Introduction}

Given their impressive performance on machine learning and pattern recognition tasks, Deep Neural Networks (\dnn{s}) have recently attracted a considerable deal of attention in several applied domains such as computer vision and natural language 
processing; see, e.g., \citet{Lecun15Nature} and references therein.

Deep Gaussian Processes \citep[\dgp{s};][]{Damianou13} are deep probabilistic models where the mapping between inputs and labels is constructed by composing functions specified in a nonparametric fashion.
From a generative perspective, \dgp{s} transform the inputs using a cascade of Gaussian Processes \citep[\gp{s};][]{Rasmussen06} such that the output of each layer of \gp{s} forms the input to the \gp{s} at the next layer.
An attractive feature of \dgp{s} is that, unlike standard \dnn{s}, their probabilistic formulation allows for a principled way to tackle quantification of uncertainty and model selection, which is desirable when employing deep models in practice. % \noteKC{To be cleared up}
\noteEB{But so do Bayesian DNNs, unclear why DGPs are different here}

The flexibility and expressive power of \dgp{s}, however, comes at the expense of having to deal with a model for which inference and predictions are inherently difficult.
%% While approximations have been developed to recover tractability in general Bayesian inference tasks \citep{Candela05,Titsias09,Hensman15,Dezfouli15}, their application to \dgp{s} remains nonetheless challenging.
This is due to the fact that the nonlinearity introduced by each layer makes it difficult to tractably propagate the uncertainty throughout the layers.
An additional complication stems from the strong coupling of the \gp{s} at all layers, which are further parameterized by covariance parameters to be optimized or inferred. \noteEB{How about the inherent complexity of GPs?}

In this paper, we develop a practical learning framework for \dgp models.
In particular, our proposal introduces two sources of approximation. % \noteKC{Generalize.}
The first is a model approximation, whereby the \gp{s} at all layers are approximated using random feature expansions \citep{Rahimi08,Gredilla10}; the second approximation relies upon stochastic variational inference to retain a probabilistic treatment of the approximate \dgp model.

%% The appeal of our proposal is that the model approximation can be tuned by selecting an appropriate number of random features, and this is dictated by constraints on running time or hardware.

%% Although our approach is amenable to any stationary covariance function, we develop it in detail for the squared exponential and arc-cosine covariance functions. 
Applying random feature expansions to \dgp{s}, we obtain \dnn{s} with low-rank weight matrices.
Feature expansions of different covariance functions result in different \dnn activation functions, namely trigonometric for the radial basis function covariance, and rectified linear unit functions for the arc-cosine covariance.
By virtue of the connection to \dnn{s}, we are able to employ scalable optimization and inference techniques that have been developed in the literature to train \dnn{s}, allowing the proposed \dgp model to scale to large data in the same way as \dnn{s}.

In order to retain a probabilistic treatment of the model when scaling to large datasets, we employ stochastic variational inference techniques.
In particular, we adapt the work on variational inference for \dnn{s} and variational autoencoders \citep{Graves11,Kingma14,Rezende14} using mini-batch-based stochastic gradient optimization for the proposed \dgp model, which can exploit GPU and distributed computing.
We implement the model in TensorFlow \citep{MartinAbadi15}, which allows us to rely on automatic differentiation during the optimization procedure.
%% The impact of the variational approximation, as opposed to characterizing the full posterior distribution over all model parameters, is the most difficult to assess.
In the supplementary material, we also illustrate the quality of our approximation by comparing the variational approximation of the proposed model with % a run of a 
the inference resulting from the application of Markov chain Monte Carlo (\mcmc) methods that we develop for two-layer \dgp regression models.

We demonstrate the effectiveness of our proposal on a variety of regression and classification problems by comparing it with other state-of-the-art approaches to infer \dgp{s} and comparable models.
The results indicate that for a given \dgp architecture, our proposal is consistently faster at achieving lower errors  compared to the competitors.
We also obtain impressive results when applying the model to large-scale problems, such as \mnisteight digit classification and the \airline dataset, which contain over $8$ and $5$ million observations, respectively.
Only very recently have there been attempts to demonstrate performance of \gp models on such large data sets \citep{Wilson16,Krauth17}, and our proposal performs at the level of these state-of-the-art \gp methods.
Crucially, we obtain these results by running our algorithm on a single machine, but we also report the performance of an asynchronous distributed version of our code in the supplementary material.
%% Such an undertaking would not have been computationally feasible using a regular \gp model, while other \dgp approaches do not converge as quickly as our technique.

%% \noteMF{Change - Furthermore, the inclusion of an asynchronous implementation of stochastic gradient optimization allows us to exploit large-scale computing facilities using distributed updates, showing that we can truly scale \dgp{s} to tractably tackle unprecedently large amounts of data.} \noteKC{Now moved to supplementary.}% \notePM{To be discussed, but I'd be careful here. Even the mnsit 8M is not that big, so we cannot really claim we learn from big data. What we do is that we exploit parallelism to lower training time, provided that our experiments really show this.}

To summarize, the contributions of this work are as follows
%% \begin{itemize}
%% \item 
(i) we propose a novel approximation of \dgp{s} based on random feature expansions;
%% \item 
(ii) we discuss the connections between the proposed approximate \dgp model and \dnn{s};
%% \item 
(iii) we compare the quality of the proposed approximation/inference framework with \mcmc techniques for a two-layer \dgp regression model;
%% \item 
(iv) we demonstrate the ability of our proposal to outperform state-of-the-art methods to carry out inference in \dgp models;
%% \item
(v) we empirically validate the superior quantification of uncertainty offered by \dgp{s} compared to \dnn{s};
%% \item  
and finally (vi) we release a TensorFlow implementation of the proposed \dgp model.
%% \item 
%% (vi) we propose an asynchronous distributed version of the code that allows us to tackle unprecedented \dgp modeling problems.
%% \end{itemize}
\noteEB{note sure code can be seen as a contribution for ICML. I'd prefer less but more concise contributions. Perhaps emphasize more on the connection to DNNs?.} 

\noteEB{May be we can focus on why DGPs are good. Flexible (non-parametric) approaches to quantifying uncertainty in DNNs. By using random features, we have a state-of-the-art way to train these models. While the resulting model is a Bayesian DNNs, we still mantain the theoretical connection with DGPs, which is important for prior setting, variable initialization and posterior analysis. In fact, we do use these tree advantages in our experiments!}

The paper is organized as follows.
The rest of this section reports the related work.
Sec.~2 introduces \dgp{s} and demonstrates how covariance functions can be approximated with random features.
In Sec.~3, we propose our construction of \dgp{s} using such approximations, and show how the resulting model can be learned using stochastic variational inference. 
Sec.~4 reports an extensive evaluation of our proposal and a thorough comparison with state-of-the-art approaches to learn \dgp{s} and \dnn{s}, while Sec.~5 concludes the paper.
\noteEB{No one really reads the paragraph above, we can get rid of it and make some room.}

